Towards AI-Powered Video Assistant Referee System (VARS) for Association Football

Over the past decade, the technology used by referees in football has improved substantially, enhancing the fairness and accuracy of decisions. This progress has culminated in the implementation of the Video Assistant Referee (VAR), an innovation that enables backstage referees to review incidents on the pitch from multiple points of view. However, the VAR is currently limited to professional leagues due to its expensive infrastructure and the lack of referees worldwide. In this paper, we present the semi-automated Video Assistant Referee System (VARS) that leverages the latest findings in multi-view video analysis. VARS sets a new state-of-the-art on the SoccerNet-MVFoul dataset, a multi-view video dataset of football fouls. Our VARS achieves a new state-of-the-art on the SoccerNet-MVFoul dataset by recognizing the type of foul in 50% of instances and the appropriate sanction in 46% of cases. Finally, we conducted a comparative study to investigate human performance in classifying fouls and their corresponding severity and compared these findings to our VARS. The results of our study highlight the potential of our VARS to reach human performance and support football refereeing across all levels of professional and amateur federations.

==> Figures/con_study_action.tex <==

\begin{figure*}
\centering
\begin{subfigure}{0.4\textwidth}
    \includegraphics[width=\textwidth]{images/ai_vs_referee_CM_action.png}
    \caption{VARS}
    \label{fig:fig_CM study action 1}
\end{subfigure}
\hfill
\begin{subfigure}{0.4\textwidth}
  \includegraphics[width=\textwidth]{images/player_vs_refereeCM_action.png}
    \caption{Players}
    \label{fig:fig_CM study action 2}
\end{subfigure}
\caption{
\textbf{Confusion matrix for the type of action classification.}
$1$: Challenge, $2$: Dive, $3$: High Leg, $4$: Holding, $5$: Elbowing, $6$: Pushing, $7$: Standing tackling, $8$: Tackling, R: Recall and P: Precision are given in percentage (\%). ``1.'' stands for 100\%.
}
 \label{fig_CM study action}
\end{figure*}


==> Figures/confOff.tex <==
 \begin{figure}[h]
 \centering
   \includegraphics[width=0.8\linewidth]{images/offence_class_SE.png}
            \caption{\textbf{Confusion matrix for the offense and severity classification.} The VARS shows good performance for the ``Offense + No card'' class. 
             For the class ``Offense + Red card'' the model cannot provide good results due to the low number of samples in the dataset.
             1: No offense, 2: Offense + No card, 3: Offense + Yellow card, 4: Offense + Red card, R: Recall and P: Precision are given in percentage (\%).} 
             \label{fig:confusion_matrix_off_SE} 
 \end{figure}

==> Figures/conf_study_off.tex <==

\begin{figure*}
\centering
\begin{subfigure}{0.4\textwidth}
    \includegraphics[width=\textwidth]{images/ai_vs_referee_CM.png}
    \caption{VARS}
    \label{fig:CM study offence 1}
\end{subfigure}
\hfill
\begin{subfigure}{0.4\textwidth}
  \includegraphics[width=\textwidth]{images/player_vs_refereeCM.png}
    \caption{Players}
    \label{fig:CM study offence 1}
\end{subfigure}
\caption{
\textbf{Confusion matrix for the offence severity classification.}
 1: No offence, 2: Offence + No card, 3: Offence + Yellow card, 4: Offence + Red card, R: Recall and P: Precision are given in percentage (\%).
}
 \label{fig:CM study offence}
\end{figure*}


==> Figures/detailed_results_survey.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=1\linewidth]{images/survey_analysis.png}
    \caption{\textbf{Average number of times each class is chosen.} While the average values for referees and players are quite similar, we observe a high standard deviation. This indicates significant variations among individuals when determining the offense and its severity. The error bars correspond to the standard deviation. 
    }
    \label{fig:detailedanalysis}
\end{figure}

==> Figures/workflow.tex <==
\begin{figure}[h]
    \centering
    \includegraphics[width=1\linewidth]{images/workflow.png}
    \caption{\textbf{Our proposed Video Assistant Referee System (VARS).} 
    1. The VARS predicts that the tackling is a `Foul' and a 'Yellow card'. 
    2. Furthermore, he automatically detects the decision of the referee. In this example, the referee shows a `Red card'. 
    3. The VARS indicates a probable `clear and obvious error’ and communicates this information to the referee, who will then decide whether to initiate a `review’. 
    4. The video clips are automatically extracted and displayed for the referee to review them in the review area.
    5. The referee can take/change/rescind his decision.}
    \label{fig:workflow}
\end{figure}

==> Tables/classes_analysis.tex <==
\begin{table*}[h]
    \centring
    \resizebox{0.92\linewidth}{!}{% <------ Don't forget this %
    \begin{tabular}{l|cc}
  &\textbf{Max} &\textbf{Attention}\\\midrule
\textbf{Tackling}         &0.16 &0.28 \\
\textbf{Stand. tackling}  &0.07 &\textbf{0.66}  \\
\textbf{High leg}         &0.13 &0.20  \\
\textbf{Holding}          &0.14 &\textbf{0.50} \\
\textbf{Pushing}          &0.18 &\textbf{0.81}  \\
\textbf{Elbowing}         &0.12 &0.37 \\
\textbf{Challenge}        &0.28 &\textbf{0.68} \\
\textbf{Dive}             &0.00 &\textbf{1.00} \\
\bottomrule
    \end{tabular}
    }
    \caption{ \textbf{Relation between the type of action and offense severity.} The distribution of the ``offense severity'' property varies significantly depending on the type of action. 
    }
    \label{tab:classesAnalysis}
\end{table*}

==> Tables/multiViews.tex <==
\begin{table}[t]
    \centering
    \resizebox{\linewidth}{!}{% <------ Don't forget this %
\begin{tabular}{l|ccccc}
\toprule
 \multirow{2}{*}{{\textbf{Performance}}} & \multicolumn{5}{c}{\textbf{Viewing Setup}} \\
 & L & R1 & L+R1 & R1+R2 & L+R1+R2 \\ \midrule
Acc$_{foul}$     &0.14   &0.53 &0.58 &\bf 0.61  &0.60\ \\
Acc$_{foul}$@2    &0.27 &0.69 &0.66 &0.68    &\bf 0.72\ \\ \midrule
Acc$_{off}$     &0.36  &0.42 &0.46 &0.50     &\bf 0.51\ \\ 
Acc$_{off}$@2    & 0.67 &0.70 &0.74  &0.75    &\bf 0.77\ \\ \bottomrule
\end{tabular}
    }
    \caption{ 
    \textbf{Single \textit{vs} multi-view classification}. We compare the performance for single vs multi-views and the influence of the type of view (Live L and replay R). We use MViT as feature extractor and attention pooling. For both tasks, the best performance is mostly obtained with all three views. \textit{foul} stands for foul classification and \textit{off} stands for offense severity classification.
   }
    \label{tab:singlemultiviewTableActionMain}
\end{table}

==> Tables/refereePlayersAnalysis.tex <==
\begin{table}[h]
    \centering
    \resizebox{1\linewidth}{!}{% <------ Don't forget this %
    \begin{tabular}{l|ccccc}
 \textbf{Nb. of different decisions} &\textbf{1} & \textbf{2} &\textbf{3} &\textbf{4} &\textbf{5} \\\midrule
\textbf{High-level referees}    &20\% &34\% &31\% & 14\% &1\% \\
\textbf{Referee talents}    &26\% &43\% &25\% &6\% &0\%  \\
\textbf{Soccer players}    &22\% &35\% &30\% &13\% &0\%  \\


\bottomrule
    \end{tabular}
    }
    \caption{ \textbf{Similarity analysis of the results for type of action classification.} For all three groups, we have a similar distribution of the same decision, two different decisions, and three different decisions.
    For 1\% of the actions, the high-level referees took five different decisions for the same action.
    }
    \label{tab:refereeanalysisType}
\end{table}

==> Tables/relationActionOffence.tex <==
\begin{table*}[h]
    \resizebox{0.92\linewidth}{!}{% <------ Don't forget this %
    \begin{tabular}{l|cccc}
  &\textbf{No offence} & \textbf{Offence + No Card} &\textbf{Offence + } \fcolorbox{black}{yellow}{\rule{0pt}{6pt}\rule{4pt}{0pt}}~~& \textbf{Offence + } \fcolorbox{black}{red}{\rule{0pt}{6pt}\rule{4pt}{0pt}}~~\\\midrule
\textbf{Tackling}         &0.16 &0.28 &\textbf{0.51} &0.05  \\
\textbf{Stand. tackling}  &0.07 &\textbf{0.66} &0.26 &0.01   \\
\textbf{High leg}         &0.13 &0.20 &\textbf{0.61} &0.06  \\
\textbf{Holding}          &0.14 &\textbf{0.50} &0.34 &0.00 \\
\textbf{Pushing}          &0.18 &\textbf{0.81} &0.01 &0.00 \\
\textbf{Elbowing}         &0.12 &0.37 &\textbf{0.49} &0.02\\
\textbf{Challenge}        &0.28 &\textbf{0.68} &0.04 &0.00\\
\textbf{Dive}             &0.00 &\textbf{1.00} &0.00 &0.00\\
\bottomrule
    \end{tabular}
    }
    \caption{ \textbf{Relation between the type of action and offense severity.} The distribution of the ``offense severity'' property varies significantly depending on the type of action. 
    }
    \label{tab:RelationTypeAndOffenceSeverity}
\end{table*}

==> acknow-declaration.tex <==
\mysection{Acknowledgement.}
This work was partly supported by the King Abdullah University of Science and Technology (KAUST) Office of Sponsored Research through the Visual Computing Center (VCC) funding and the SDAIA-KAUST Center of Excellence in Data Science and Artificial Intelligence (SDAIA-KAUST AI). 
A. Cioppa is funded by the F.R.S.-FNRS, Belgium.

\section*{Declarations} 
\mysection{Availability of data and code.} The data will be available after publication \url{https://github.com/SoccerNet/VARS}.

\mysection{Ethics approval.} The Ethics Committee of the FPLSE at the University of Li{\`e}ge issued a favorable opinion on 2/06/2023 for our human study (reference 2223-080/5624).

\mysection{Conflict of interest.} The authors declare no conflict of interest.

\mysection{Open Access.} This article is licensed under a Creative Commons Attribution 4.0 International License, which permits use, sharing, adaptation, distribution, and reproduction in any medium or format, as long  as you give appropriate credit to the original author(s) and the source,  provide a link to the Creative Commons license, and indicate if changes were made. The images or other third-party material in this article are included in the article's Creative Commons license, unless indicated otherwise in a credit line to the material. If material is not included in the article's Creative Commons license and your intended use is not permitted by statutory regulation or exceeds the permitted use, you will need to obtain permission directly from the copyright holder. To view a copy of this license, visit \url{http://creativecommons.org/licenses/by/4.0/}.


